Ground-Optimized 4D Radar-Inertial Odometry via Continuous Velocity Integration using Gaussian Process

Radar ensures robust sensing capabilities in adverse weather conditions, yet challenges remain due to its high inherent noise level. Existing radar odometry has overcome these challenges with strategies such as filtering spurious points, exploiting Doppler velocity, or integrating with inertial measurements. This paper presents two novel improvements beyond the existing radar-inertial odometry: ground-optimized noise filtering and continuous velocity preintegration. Despite the widespread use of ground planes in LiDAR odometry, imprecise ground point distributions of radar measurements cause naive plane fitting to fail. Unlike plane fitting in LiDAR, we introduce a zone-based uncertainty-aware ground modeling specifically designed for radar. Secondly, we note that radar velocity measurements can be better combined with IMU for a more accurate preintegration in radar-inertial odometry. Existing methods often ignore temporal discrepancies between radar and IMU by simplifying the complexities of asynchronous data streams with discretized propagation models. Tackling this issue, we leverage GP and formulate a continuous preintegration method for tightly integrating 3-DOF linear velocity with IMU, facilitating full 6-DOF motion directly from the raw measurements. Our approach demonstrates remarkable performance (less than 1% vertical drift) in public datasets with meticulous conditions, illustrating substantial improvement in elevation accuracy. The code will be released as open source for the community: https://github.com/wooseongY/Go-RIO.

==> note.tex <==
# Free Notes


% %FIGURE
% \begin{figure}[!t]
%     \centering
%    % \vspace{-1mm}
%     \subfloat[Overlap of two images\label{fig:feature_overlap1}]{
% 		\includegraphics[height=0.48\columnwidth]{./figs/overlap.png}
%     }
%     \subfloat[Revloution scan delay\label{fig:feature_overlap2}]{
% 		\includegraphics[height=0.48\columnwidth]{./figs/overlap2.png}
% 	}\\
%     \subfloat[Contour and nearest point extraction\label{fig:feature_contour}]{
% 		\includegraphics[width=0.98\columnwidth]{./figs/features.pdf}
% 	}
%     \vspace{-1mm}
%     \caption{(a) In our dataset, certain regions remain un-updated due to the low update rate. An accumulation in these overlapping areas could lead to unexpected convergence behaviors. (b) Given that radar imagery inherently constitutes scan-rotated images, there exists a discrepancy between the commencement and conclusion of the scans, primarily attributed to temporal lags. This discrepancy is especially pronounced during sharp rotational movements. (c) Initially, we delineate the contour, subsequently identifying proximal points to ensure consideration extends beyond just the central points.}
%     \label{fig:feature}
%     \vspace{-5mm}
% \end{figure}


% %FIGURE
% \begin{figure}[!t]
%     \centering
%    % \vspace{-1mm}
%     \includegraphics[width=0.98\columnwidth]{./figs/fig3.pdf}
%     \vspace{-1mm}
%     \caption{Concept of the LodeStar Descriptor. From the primary radar imagery, we compute a radial intensity vector for every $\theta$. Each of these vectors is subsequently integrated to constitute a column within the integrated radial intensity matrix. By iterating this process over a period of 2$\pi$, we synthesize the final descriptor.}
%     \label{fig:lodestar}
%     \vspace{-5mm}
% \end{figure}


root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-48-03_minmax/recall_rates.csv 
STHEREO-SNU, 56.73, 74.61, 80.08, 84.90
STHEREO-valley, 83.60, 96.46, 98.71, 99.36
vivid-urban, 92.22, 98.13, 99.22, 99.69
vivid-city, 92.02, 96.55, 98.17, 98.99

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-49-24_histeq/recall_rates.csv 
STHEREO-SNU, 63.02, 79.35, 84.41, 88.33
STHEREO-valley, 75.88, 89.39, 94.53, 96.14
vivid-urban, 91.91, 98.29, 98.91, 99.69
vivid-city, 89.25, 97.84, 98.78, 99.19

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-50-31_minmax_gridwise_8x8/recall_rates.csv 
STHEREO-SNU, 53.55, 75.02, 81.31, 86.69
STHEREO-valley, 50.80, 71.38, 76.85, 81.99
vivid-urban, 88.49, 96.58, 98.76, 99.53
vivid-city, 91.62, 96.08, 97.50, 98.65

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-51-45_minmax_gridwise_message_passing_8x8_mean_3/recall_rates.csv 
STHEREO-SNU, 61.80, 79.51, 85.22, 89.80
STHEREO-valley, 87.78, 97.43, 98.71, 99.04
vivid-urban, 93.78, 98.44, 99.07, 99.84
vivid-city, 92.97, 96.08, 97.57, 98.51

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-53-10_minmax_gridwise_message_passing_8x8_mean_5/recall_rates.csv 
STHEREO-SNU, 60.33, 77.80, 81.80, 87.27
STHEREO-valley, 90.03, 96.78, 98.07, 99.36
vivid-urban, 94.40, 99.22, 99.38, 99.84
vivid-city, 91.35, 96.42, 97.70, 98.65

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-54-42_minmax_gridwise_message_passing_16x16_mean_3/recall_rates.csv 
STHEREO-SNU, 65.71, 80.24, 84.33, 89.06
STHEREO-valley, 76.21, 91.00, 95.18, 96.78
vivid-urban, 92.07, 97.51, 99.07, 100.00
vivid-city, 90.40, 96.35, 97.77, 98.65

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-55-56_minmax_gridwise_message_passing_16x16_mean_5/recall_rates.csv 
STHEREO-SNU, 59.67, 77.55, 83.51, 88.24
STHEREO-valley, 76.85, 90.03, 95.50, 97.43
vivid-urban, 89.27, 97.20, 99.07, 99.84
vivid-city, 90.94, 95.47, 97.63, 98.58

root@oem-System-Product-Name:/home/hj/Backup/test# cat 2023-09-11_02-57-11_minmax_gridwise_message_passing_16x16_mean_7/recall_rates.csv 
STHEREO-SNU, 60.90, 78.94, 84.90, 88.82
STHEREO-valley, 78.46, 93.89, 97.43, 99.36
vivid-urban, 90.82, 97.67, 99.38, 99.84
vivid-city, 90.80, 96.15, 97.90, 98.99


==> tab/MSC_tab.tex <==
\begin{table}[t]
    \scriptsize
    \caption{\ac{ATE} Evaluation results in MSC-RAD4R}
    \vspace{-1mm}
    \label{table:msc}
    \centering
    \resizebox{0.45\textwidth}{!}{%
    \begin{tabular}{ccccccc}
    \toprule
    & \begin{tabular}[c]{@{}c@{}}4DRadarSLAM\end{tabular} & \begin{tabular}[c]{@{}c@{}}EKF-RIO \end{tabular} & BCV & DeRO & Ours \\
    \midrule[1pt]
    \multicolumn{1}{c|}{\multirow{1}{*}{ {\texttt{URBAN\_A0}}}}  & 16.097 & 18.638 & \textit{2.677} & 12.317 & \textbf{1.757} \\
    \midrule
    \multicolumn{1}{c|}{\multirow{1}{*}{ {\texttt{LOOP\_A0}}}}  & 110.269 & \textit{96.662} & 120.297 & 149.277 & \textbf{16.752} \\
    \midrule
    \multicolumn{1}{c|}{\multirow{1}{*}{ {\texttt{LOOP\_B0}}}}  & 88.228 & 159.662 & 130.256 & \textit{39.620} & \textbf{9.884} \\
    \midrule
    \multicolumn{1}{c|}{\multirow{1}{*}{ {\texttt{LOOP\_C0}}}}  & \textit{14.333} & 176.106& 81.444 & 51.058 & \textbf{6.450} \\
    \midrule
    \multicolumn{1}{c|}{\multirow{1}{*}{ {\texttt{LOOP\_D0}}}}  & \textit{19.984} & 26.895 & 75.382 & 46.708 & \textbf{4.280}\\
    \midrule
    \multicolumn{1}{c|}{\multirow{1}{*}{ {\texttt{LOOP\_E0}}}}  & \textit{56.347} & 196.652	& 95.018 & 186.376 & \textbf{35.266} \\
    \midrule
    \multicolumn{1}{c|}{\multirow{1}{*}{ {\texttt{RURAL\_A2}}}}  & 33.256 & 278.788 & \textit{19.423} & 263.003 & \textbf{9.480} \\
    \midrule
    \multicolumn{1}{c|}{\multirow{1}{*}{ {\texttt{RURAL\_B2}}}}  & 24.251 & 251.471 & \textit{14.256} & 73.784 & \textbf{10.927} \\
    \bottomrule
    \end{tabular}}    
    \vspace{-4mm}
\end{table}

==> tab/NTU_tab.tex <==
\begin{table}[t]
    \scriptsize
    \caption{NTU4DRadLM Dataset}
    \vspace{-1mm}
    \label{table:ntu}
    \centering
    \resizebox{0.45\textwidth}{!}{%
    \begin{tabular}{ccccccc}
    \toprule
    & & \begin{tabular}[c]{@{}c@{}}4DRadarSLAM\end{tabular} & \begin{tabular}[c]{@{}c@{}}EKF-RIO \end{tabular} & BCV & DeRO & Ours \\
    \midrule[1pt]
    \multicolumn{1}{c|}{\multirow{3}{*}{ \rotatebox{90}{\texttt{cp}}}} & \multicolumn{1}{c|}{ATE} 
     & \textit{0.768} & 6.241 & 3.163 & 4.910 & \textbf{0.699} \\
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{RPE$_r$}
     & \textit{1.107} & 1.806  & 1.232 & 1.625 & \textbf{0.722} \\
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{RPE$_t$} 
     & 0.106 & 0.298 & \textit{0.096} & 0.112 & \textbf{0.085} \\
    \midrule
    \multicolumn{1}{c|}{\multirow{3}{*}{ \rotatebox{90}{\texttt{nyl}}}} & \multicolumn{1}{c|}{ATE} 
     & \textit{7.574} & 58.913  & 41.002 & 48.275 & \textbf{5.009} \\
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{RPE$_r$}
     & 1.106 & 1.864 & \textbf{0.949} & 1.610 & \textit{1.003}  \\
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{RPE$_t$}
     & 0.178 & 0.423 & \textit{0.142} & 0.318 & \textbf{0.116} \\
    \midrule
    \multicolumn{1}{c|}{\multirow{3}{*}{ \rotatebox{90}{\texttt{loop2}}}} & \multicolumn{1}{c|}{ATE}
     & \textit{131.948} & 436.262 & 222.182 & 438.643 & \textbf{89.209} \\
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{RPE$_r$}
     & 0.751 & 1.179 & \textit{0.564} & 0.880 & \textbf{0.547} \\
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{RPE$_t$}
     & 0.450 & 1.750 & \textit{0.368} & 2.059 & \textbf{0.338} \\
    \midrule
    \multicolumn{1}{c|}{\multirow{3}{*}{ \rotatebox{90}{\texttt{loop3}}}} & \multicolumn{1}{c|}{ATE}
     & \textbf{26.755} & 181.422 & 231.449 & 146.659 & \textit{42.864} \\
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{RPE$_r$}
     & 0.562 & 0.596 & 0.537 & \textit{0.524} & \textbf{0.384} \\
    \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{RPE$_t$}
     & 0.472 & 1.307 & 0.546 & \textit{0.373} & \textbf{0.365} \\
    \bottomrule
    \end{tabular}}
    \captionsetup{font=footnotesize}
    \caption*{\raggedright \footnotesize $\quad$The best are in \textbf{bold}, and the second-best are shown in \textit{italics}.}
    \vspace{-6mm}
\end{table}

==> tab/RPE.tex <==
\begin{table}[t]
% \resizebox{\linewidth}{!}
\scriptsize
\centering
\caption{Translational and Rotational Relative Pose Error (Trans(m)/Rot(deg)) in NTU4DRadLM}
\vspace{-1mm}
\label{tab:result_rpe}
\resizebox{0.45\textwidth}{!}{
\begin{tabular}{l|cccc}
\hline
\textbf{Method} & \textbf{cp} & \textbf{nyl} & \textbf{loop2} & \textbf{loop3} \\ \hline\hline
4DRadarSLAM & 0.106/1.107 & 0.178/1.106 & 0.745/0.751 & 0.472/0.562 \\ 
EKF-RIO     & 0.298/1.806 & 0.423/1.864 & 1.750/1.179 & 1.307/0.596 \\
BCV         & 0.096/1.232 & 0.142/\textbf{0.949} & 0.368/0.564 & 0.546/0.537 \\ 
DeRO        & 0.112/1.625 & 0.318/1.610 & 2.059/0.368 & 0.373/0.524 \\ 
Proposed    & \textbf{0.085}/\textbf{0.722} & \textbf{0.116}/1.003 & \textbf{0.338}/\textbf{0.547} & \textbf{0.365}/\textbf{0.384} \\ \hline
\end{tabular}}
\vspace{-2mm}
\end{table}
